Crucible: Graphical Test Cases for Alloy Models

Alloy is a declarative modeling language that is well suited for verifying system designs. Alloy models are automatically analyzed using the Analyzer, a toolset that helps the user understand their system by displaying the consequences of their properties, helping identify any missing or incorrect properties, and exploring the impact of modifications to those properties. To achieve this, the Analyzer invokes off-the-shelf SAT solvers to search for scenarios, which are assignments to the sets and relations of the model such that all executed formulas hold. To help write more accurate software models, Alloy has a unit testing framework, AUnit, which allows users to outline specific scenarios and check if those scenarios are correctly generated or prevented by their model. Unfortunately, AUnit currently only supports textual specifications of scenarios. This paper introduces Crucible, which allows users to graphically create AUnit test cases. In addition, Crucible provides automated guidance to users to ensure they are creating well structured, valuable test cases. As a result, Crucible eases the burden of adopting AUnit and brings AUnit test case creation more in line with how Alloy scenarios are commonly interacted with, which is graphically.

==> figures/addr.tex <==
\begin{scriptsize}
\begin{Verbatim}[]
\Blue{abstract sig} Listing \{\}
\Blue{sig} Address \Blue{extends} Listing \{\}
\Blue{sig} Name \Blue{extends} Listing \{\}
\Blue{sig} Book \{
  entry: \Blue{set} Name, 
  listed: entry ->\Blue{set} Listing
\}
\Blue{fun} lookup [b: Book, n: Name] : \Blue{set} Listing \{n.^(b.listed)\}

\Green{// A name entry maps to at most one name or address.}
\Blue{fact} \{ \Blue{all} b:Book | \Blue{all} n:b.entry | \Blue{lone} b.listed[n] \}
\Green{// All names reachable from any name entry in the book are themselves entries.}
\Blue{fact} \{ \Blue{all} b:Book | \Blue{all} n,l:Name | l \Blue{in} lookup[b,n] \Red{implies} l \Blue{in} b.entry \}
\Green{// Acyclic}
\Blue{fact} \{ \Blue{all} b:Book | \Blue{all} n:b.entry | \Blue{not} n \Blue{in} lookup[b,n] \}

\Blue{assert} lookupEndsInAddr \{
  \Blue{all} b:Book | \Blue{all} n:b.entry | \Blue{some} (lookup[b,n]&Address)
\}
\Blue{check} lookupEndsInAddr \Blue{for} 4

\Blue{val} AddrTest1 \{
  \Blue{some disj} Address0: Address \{ \Blue{some disj} Name0, Name1: Name \{ \Blue{some disj} Name0, Name1, Address0: Listing \{
  \Blue{some disj} Book0, Book1, Book2: Book \{
    Address = Address0
    Name = Name0 + Name1
    Listing = Name0 + Name1 + Address0
    Book = Book0 + Book1 + Book2
    entry = Book0->Name0 + Book0->Name1 + Book1->Name0 + Book1->Name1 + Book2->Name0 + Book2->Name1
    listed = Book0->Name0->Address0 + Book0->Name1->Name0 + Book0->Name1->Address0 + Book1->Name0->Address0 + 
      Book1->Name1->Name0 + Book1->Name1->Address0 + Book2->Name0->Address0 + Book2->Name1->Name0 + Book2->Name1->Address0
  \}\}\}\}
\}
\LightBlue{@Test} AddrTest1: \Blue{run} AddrTest1 
\end{Verbatim}
\end{scriptsize}

==> figures/alloy.tex <==
\usetikzlibrary{shapes.geometric, arrows}
\tikzstyle{arrow} = [line width=1.5pt,->,>=stealth]
\tikzstyle{darrow} = [line width=1.5pt,<->,>=stealth]
\tikzstyle{NodeAtom} = [rectangle, minimum width=.75cm, minimum height=.75cm, text centered, draw=black, fill=yellow!75!orange]
\tikzstyle{ListAtom} = [rectangle, minimum width=.75cm, minimum height=.75cm, text centered, draw=black, fill=orange!75!yellow]

\begin{figure*}
    \centering
\begin{tabular}[t]{c|c|c|c}
\footnotesize (a) & \footnotesize (b) & \footnotesize (c) & \footnotesize (d)\\
\begin{minipage}[t]{.6\columnwidth}
\scriptsize
\begin{Verbatim}[]
1. \Blue{one sig} List \{header: \Blue{lone} Node\}
2. \Blue{sig} Node \{link: \Blue{lone} Node\} 
3. \Blue{pred} acyclic \{
4.   \Blue{all} n : List.header.*link\{
5.     n !\Blue{in} n.^link \}
6. \}
7. \Blue{run} \{acyclic\} \Blue{for} 3
\end{Verbatim}

\end{minipage}

&
\begin{minipage}[t]{.15\columnwidth}
\begin{center}
\begin{tikzpicture}[baseline,node distance=1.5cm]
\node (L0) [ListAtom] {\textbf{L0}};
\begin{scope}[red]
\end{scope}[red]
\end{tikzpicture}
\end{center}
\end{minipage}

&

\begin{minipage}[t]{.2\columnwidth}
\begin{center}
\begin{tikzpicture}[baseline,node distance=1.5cm]
\node (L0) [ListAtom] {\textbf{L0}};
\node (N0) [NodeAtom, below of=L0] {\textbf{N0}};
\begin{scope}[red]
\draw [arrow] (L0) -- node[anchor=west] {\textbf{header}} (N0);
\end{scope}[red]
\end{tikzpicture}
\end{center}
\end{minipage}

&

\begin{minipage}[t]{.45\columnwidth}
\begin{center}
\begin{tikzpicture}[baseline,node distance=1.5cm]
\node (L0) [ListAtom] {\textbf{L0}};
\node (N0) [NodeAtom, below of=L0] {\textbf{N0}};
\node (N1) [NodeAtom, right of=N0] {\textbf{N1}};
\begin{scope}[red]
\draw [arrow] (L0) -- node[anchor=west] {\textbf{header}} (N0);
\end{scope}[red]
\begin{scope}[brown]
%\draw [arrow] (N0) -- node[anchor=north] {\textbf{link}} (N1);
\draw [arrow] (N1) edge [loop right,line width=1.5pt] node {\textbf{link}} (N1);
\end{scope}[brown]
\end{tikzpicture}
\end{center}
\end{minipage}
\end{tabular}
    \caption{Alloy Model of a Singly-Linked List}
    \label{fig:alloy}
\end{figure*}

==> figures/arr.tex <==
\begin{scriptsize}
\begin{Verbatim}[]
\Blue{sig} Element \{\}

\Blue{one sig} Array \{
  i2e: \Blue{Int} -> Element,  \Green{// Maps indexes to elements.}
  length: \Blue{Int}
\}

\Blue{fact} \{
  Element = Array.i2e[Int] \Green{//Reachable}
  \Green{// All indexes should be greater than or equal to 0 and less than the array length}
  \Blue{all} i:Array.i2e.Element | i >= 0 \Blue{and} i < Array.length
  \Green{// Array length should be greater than equal to 0}
  Array.length >= 0
\}

\Blue{pred} NoConflict() \{ \Green{// Each index maps to at most on element}
  \Blue{all} i:Array.i2e.Element | #Array.i2e[i] <= 1
\}
\Blue{run} NoConflict \Blue{for} \Red{3}

\Blue{val} test1 \{
  \Blue{some disj} Element0, Element1: Element \{
  \Blue{some disj} Array0: Array \{
    Element = Element0 + Element1
    Array = Array0
    i2e = Array0->0->Element1 + Array0->1->Element0 + Array0->2->Element0 + Array0->3->Element1 + 
          Array0->4->Element0 + Array0->5->Element0
    length = Array0->6
    NoConflict[]
  \}\}
\}
\LightBlue{@Test} test1: \Blue{run} test1 
\end{Verbatim}
\end{scriptsize}

==> figures/grade.tex <==
\begin{scriptsize}
\begin{Verbatim}[]
\Blue{abstract sig} Person \{\}
\Blue{sig} Student \Blue{extends} Person \{\}
\Blue{sig} Professor \Blue{extends} Person \{\}
\Blue{sig} Class \{
  assistant_for: \Blue{set} Student, 
  instructor_of: \Blue{one} Professor
\}
\Blue{sig} Assignment \{
  associated_with: \Blue{one} Class,
  assigned_to: \Blue{some} Student
\}

\Blue{pred} PolicyAllowsGrading(s: Person, a: Assignment) \{
  s \Blue{in} a.associated_with.assistant_for \Blue{or} s \Blue{in} a.associated_with.instructor_of
  s !\Blue{in} a.assigned_to
\}

\Blue{val} GradeTest1 \{
  \Blue{some disj} Student0, Student1: Student\{ \Blue{some disj} Professor0: Professor\{ \Blue{some disj} Student0, Student1, Professor0: Person\{ 
  \Blue{some disj} Class0, Class1, Class2: Class\{ \Blue{some disj} Assignment0, Assignment1, Assignment2: Assignment\{
    Student = Student0 + Student1
    Professor = Professor0
    Person = Student0 + Student1 + Professor0
    Class = Class0 + Class1 + Class2
    assistant_for = Class0->Student1 + Class1->Student0 + Class1->Student1 + Class2->Student0 + Class2->Student1
    instructor_of = Class0->Professor0 + Class1->Professor0 + Class2->Professor0
    Assignment = Assignment0 + Assignment1 + Assignment2
    associated_with = Assignment0->Class2 + Assignment1->Class1 + Assignment2->Class0
    assigned_to = Assignment0->Student1 + Assignment1->Student0 + Assignment2->Student1
    PolicyAllowsGrading[Professor0,Assignment2]
  \}\}\}\}\}
\}
\end{Verbatim}
\end{scriptsize}


==> figures/systemArchitecture.tex <==
\usetikzlibrary{shapes.geometric,shapes.symbols,fit,positioning,shadows}
% https://tex.stackexchange.com/a/12039/121799

\begin{figure*}
    \centering
    \caption{System Architecture Diagram - \tool{}}
    \label{fig:alloy}
\begin{tikzpicture}
\node[regular polygon,regular polygon sides=6,fill=teal,text=white](Alloy) {Alloy};

\node[ above=of Alloy, cylinder, cylinder uses custom fill, cylinder end fill=blue!25,
cylinder body fill=blue!50,shape border rotate=90,text=white,
aspect=0.4,minimum width=1cm,minimum height=1.4cm,](Sqlite){SQLite};

\node[right=of Sqlite,regular polygon,regular polygon sides=4,fill=orange,text=white] (Main) {ipcMain};

\node[right=of Main,regular polygon,regular polygon sides=4,fill=orange,text=white] (Render) {ipcRenderer};

\node[draw,dashed,rounded corners,inner
xsep=10pt,label={above:{Electron}}, fit=(Main) (Render)](Electron){};

\node[right=1cm of Render,circle,fill=cyan,text=white] (React) {React};

\node[draw,rounded corners,inner
sep=10pt,minimum height=6cm,label={above:{Front-End}}, fit=(Render) (React)](Frontend){};

\node[draw,rounded corners,inner
sep=10pt,minimum height=6cm,label={above:{Back-End}}, fit=(Sqlite) (Alloy) (Main)](Backend){};

\draw[-latex] (Render) -> (Main);
\draw[-latex] (Main) -> (Render);
\draw[-latex] (Main) -> (Sqlite);
\draw[-latex] (Sqlite) -> (Main);
\draw[-latex] (Main) -> (Alloy);
\draw[-latex] (Alloy) -> (Main);
\draw[-latex] (Render) -> (React);
\draw[-latex] (React) -> (Render);

% 
\end{tikzpicture}
\end{figure*}

